Energy Aware Deep Reinforcement Learning Scheduling for Sensors Correlated in Time and Space

Millions of battery-powered sensors deployed for monitoring purposes in a multitude of scenarios, e.g., agriculture, smart cities, industry, etc., require energy-efficient solutions to prolong their lifetime. When these sensors observe a phenomenon distributed in space and evolving in time, it is expected that collected observations will be correlated in time and space. In this paper, we propose a Deep Reinforcement Learning (DRL) based scheduling mechanism capable of taking advantage of correlated information. We design our solution using the Deep Deterministic Policy Gradient (DDPG) algorithm. The proposed mechanism is capable of determining the frequency with which sensors should transmit their updates, to ensure accurate collection of observations, while simultaneously considering the energy available. To evaluate our scheduling mechanism, we use multiple datasets containing environmental observations obtained in multiple real deployments. The real observations enable us to model the environment with which the mechanism interacts as realistically as possible. We show that our solution can significantly extend the sensors' lifetime. We compare our mechanism to an idealized, all-knowing scheduler to demonstrate that its performance is near-optimal. Additionally, we highlight the unique feature of our design, energy-awareness, by displaying the impact of sensors' energy levels on the frequency of updates.

==> src/sections/section_min_power_consumption.tex <==
We illustrate the lifetime maximization problem in our system as follows:

\begin{subequations}
	\begin{equation}
	\operatorname{max} \phantom{,} \mathcal{L}_{n} \phantom{,} \operatorname{by} \phantom{,} \operatorname{max} \phantom{,} T_{n},
	\end{equation}
	\begin{equation}
	\operatorname{subject} \phantom{,} \operatorname{to:} \phantom{,} \varepsilon \big (\bm{x}_{n},t| \theta_1(t_k), \theta_2(t_k) \big ) \leq \varepsilon_{target}(t_j) \phantom{,},
	\end{equation}
	\begin{equation}
	\operatorname{and} \phantom{,} \mathbb{E}_{n} \sim  \sum_{i=1}^{N} \frac{\mathbb{E}_{i}}{N},
	\end{equation}
	\begin{equation}
	\operatorname{for} \phantom{,} \operatorname{each} \phantom{,}  n=1, \ldots, N.
	\end{equation}
\end{subequations}
\alex{there is no mention of the sensor wake-sleep schedule in the optimisation problem}

The $\varepsilon_{target} \in (0,1]$, i.e., pre-specified boundary dictated by services,can change at every time instance $t_{j}, j=1, \ldots, J$, $t_j \in \left[0, t\right]$. Additionally, the scaling parameters change at every time instance $t_{k}$. At every such change, the system has to determine new update times for $N$ sensors, each relying on $M$ past observations, and wait until the sensor wakes up to set the new optimal update time. 

When determining the optimal updating policy, the system faces a significant restriction due to dynamic changes in the estimation error. Any new observation can alter the scaling parameters in the covariance model thus causing a change in the estimation error value independently of selected update times. As soon as the scaling parameters change, the system would have to determine the new update time. However, due to the use of sleep mode, the system has to wait until the sensor wakes-up to set the new optimal update time. That may cause a problem, as the determined update time may not be optimal at the time the sensor transmits again. Meaning that the system is collecting inaccurate observations or the sensor is shortening its lifetime without any gain for the system. Furthermore, interaction between sensors and the rest of the \ac{iot} network adds to the system dynamics. A service relying on observations collected may change the $\varepsilon_{target}$ depending on the user requirements. For example, traffic sensors in a smart city should transmit more often when traffic is congested than during off-peak hours when roads are empty. Additionally, the determined update time also depend on the available energy, adding another layer of complexity when searching for the optimal update time. 


We propose an updating mechanism using \ac{rl} \cite{sutton1998reinforcement} capable finding a way to set sources updates to prolong every sensor lifetime on the long-term.... \alex{where did the rest of the sentence go :) }

In such a system, as we presented in this section, the update time has to be constantly adapted to the ever-changing environment. To that end, we employ \ac{rl} \cite{sutton1998reinforcement} to design an adaptable updating mechanism.




In our system, interactions between sensors are non-trivial, as every received observation reduces the value of estimation error at every observation point. Changing update time at one sensor has a cascading effect on every other sensor in the system, e.g., reducing update time for one sensor leads to an update time increase on other sensors. Furthermore, any new observation alters the scaling parameters in the covariance model thus causing a change in the estimation error value. The faster the sensors are transmitting new observations, the faster will the scaling parameters alter. Additionally, sensors may change their update times depending on requirements of services relying on observations collected. For example, in a smart factory,  sensors should transmit more often on working days than during the weekend. The decision on when the sensor should transmit next also depends on the available energy.



A traditional optimisation approach would force the system to find a new optimal solution whenever a sensor sends a  new observation. Moreover, if sensors are transmitting new observations with a high frequency, e.g., in industrial \ac{iot}, the system might receive a new observation before even finding an optimal solution. To address this issue we turn to \ac{rl} \cite{sutton1998reinforcement} and translate the problem into a decision-making process. 


under which conditions should take a specific action. In our case, the relevant sensors conditions are their update time, available energy, and the value of estimation error at their location. The goal of learning is to determine the update time with which the sensors should send their observations and simultaneously prolong their lifetime.


Connection to next section, kinda an additional short paragraph
In the next s, we model the system using \ac{mdp} \cite{MDP_survey} to solve above-described problem using \ac{rl} and describe an updating mechanism that enables the system to learn when should a sensor transmit its next observation.


